Facet-Aware Multi-Head Mixture-of-Experts Model with Text-Enhanced Pre-training for Sequential Recommendation

Sequential recommendation (SR) systems excel at capturing users' dynamic preferences by leveraging their interaction histories. Most existing SR systems assign a single embedding vector to each item to represent its features, adopting various models to combine these embeddings into a sequence representation that captures user intent. However, we argue that this representation alone is insufficient to capture an item's multi-faceted nature (e.g., movie genres, starring actors). Furthermore, users often exhibit complex and varied preferences within these facets (e.g., liking both action and musical films within the genre facet), which are challenging to fully represent with static identifiers. To address these issues, we propose a novel architecture titled Facet-Aware Multi-Head Mixture-of-Experts Model for Sequential Recommendation (FAME). We leverage sub-embeddings from each head in the final multi-head attention layer to predict the next item separately, effectively capturing distinct item facets. A gating mechanism then integrates these predictions by dynamically determining their importance. Additionally, we introduce a Mixture-of-Experts (MoE) network within each attention head to disentangle varied user preferences within each facet, utilizing a learnable router network to aggregate expert outputs based on context. Complementing this architecture, we design a Text-Enhanced Facet-Aware Pre-training module to overcome the limitations of randomly initialized embeddings. By utilizing a pre-trained text encoder and employing an alternating supervised contrastive learning objective, we explicitly disentangle facet-specific features from textual metadata (e.g., descriptions) before sequential training begins. This ensures that the item embeddings are semantically robust and aligned with the downstream multi-facet framework.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> maintable.tex <==
%auto-ignore
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[t]
\small
\centering
\caption{Performance comparison of different methods on top-$k$ recommendation}
\label{tab: mainresults}
\begin{tabular}{clcccccccccccc}
\toprule
Dataset                 & Metric  & GRU4Rec & SASRec       & BERT4Rec     & CORE   & CL4SRec & ICLRec       & DuoRec       & A-Mixer & MSGIFSR & MiaSRec      & FAME            & Improv. \\
\midrule
\multirow{6}{*}{Beauty} & HR@5    & 0.0408  & 0.0508       & 0.0510       & 0.0331 & 0.0623 & {\ul 0.0664} & 0.0504       & 0.0507  & 0.0518  & 0.0524       & \textbf{0.0710} & 6.9\%  \\
                        & HR@10   & 0.0623  & 0.0761       & 0.0745       & 0.0664 & 0.0877 & {\ul 0.0918} & 0.0691       & 0.0752  & 0.0771  & 0.0795       & \textbf{0.0978} & 6.2\%  \\
                        & HR@20   & 0.0895  & 0.1057       & 0.1075       & 0.1071 & 0.1195 & {\ul 0.1252} & 0.0912       & 0.1033  & 0.1105  & 0.1125       & \textbf{0.1345} & 7.4\%  \\
                        & NDCG@5  & 0.0273  & 0.0318       & 0.0343       & 0.0164 & 0.0440 & {\ul 0.0480} & 0.0363       & 0.0350  & 0.0344  & 0.0362       & \textbf{0.0508} & 5.8\%  \\
                        & NDCG@10 & 0.0342  & 0.0400       & 0.0419       & 0.0271 & 0.0521 & {\ul 0.0562} & 0.0424       & 0.0421  & 0.0429  & 0.0449       & \textbf{0.0593} & 5.5\%  \\
                        & NDCG@20 & 0.0410  & 0.0474       & 0.0502       & 0.0373 & 0.0601 & {\ul 0.0646} & 0.0479       & 0.0504  & 0.0508  & 0.0532       & \textbf{0.0687} & 6.3\%  \\
\hline
\multirow{6}{*}{Sports} & HR@5    & 0.0210  & 0.0266       & 0.0252       & 0.0150 & 0.0338 & {\ul 0.0384} & 0.0225       & 0.0217  & 0.0268  & 0.0270       & \textbf{0.0400} & 4.2\%  \\
                        & HR@10   & 0.0339  & 0.0412       & 0.0395       & 0.0342 & 0.0498 & {\ul 0.0543} & 0.0327       & 0.0321  & 0.0425  & 0.0435       & \textbf{0.0580} & 6.8\%  \\
                        & HR@20   & 0.0527  & 0.0618       & 0.0607       & 0.0609 & 0.0723 & {\ul 0.0753} & 0.0476       & 0.0469  & 0.0634  & 0.0651       & \textbf{0.0820} & 8.9\%  \\
                        & NDCG@5  & 0.0136  & 0.0158       & 0.0166       & 0.0072 & 0.0235 & {\ul 0.0266} & 0.0161       & 0.0165  & 0.0171  & 0.0180       & \textbf{0.0277} & 4.1\%  \\
                        & NDCG@10 & 0.0178  & 0.0205       & 0.0212       & 0.0134 & 0.0287 & {\ul 0.0317} & 0.0193       & 0.0188  & 0.0221  & 0.0233       & \textbf{0.0337} & 6.3\%  \\
                        & NDCG@20 & 0.0225  & 0.0256       & 0.0265       & 0.0201 & 0.0344 & {\ul 0.0370} & 0.0231       & 0.0235  & 0.0279  & 0.0288       & \textbf{0.0402} & 8.6\%  \\
\hline
% \multirow{6}{*}{Steam}  & HR@5    & 0.3348  & 0.3374       & 0.1529       & 0.2513 & 0.1173 & 0.1429       & 0.1511       & 0.3356  & 0.3295  & {\ul 0.3401} & \textbf{0.3561} & 4.7\%  \\
%                         & HR@10   & 0.4046  & {\ul 0.4069} & 0.2191       & 0.2848 & 0.1721 & 0.2066       & 0.2147       & 0.3913  & 0.3847  & 0.4027       & \textbf{0.4244} & 4.3\%  \\
%                         & HR@20   & 0.4877  & {\ul 0.4890} & 0.3016       & 0.3338 & 0.2448 & 0.2866       & 0.2931       & 0.4679  & 0.4636  & 0.4798       & \textbf{0.5144} & 5.2\%  \\
%                         & NDCG@5  & 0.2752  & 0.2774       & 0.1051       & 0.2245 & 0.0796 & 0.0967       & 0.1035       & 0.2751  & 0.2697  & {\ul 0.2839} & \textbf{0.2978} & 4.9\%  \\
%                         & NDCG@10 & 0.2977  & 0.2999       & 0.1264       & 0.2353 & 0.0973 & 0.1172       & 0.1240       & 0.2965  & 0.2884  & {\ul 0.3041} & \textbf{0.3175} & 4.4\%  \\
%                         & NDCG@20 & 0.3186  & 0.3206       & 0.1472       & 0.2477 & 0.1156 & 0.1374       & 0.1437       & 0.3197  & 0.3101  & {\ul 0.3235} & \textbf{0.3400} & 5.1\%  \\
\multirow{6}{*}{Toys}   & HR@5    & 0.0369  & 0.0489       & 0.0464       & 0.0338 & 0.0658 & {\ul 0.0792} & 0.0481       & 0.0565  & 0.0576  & 0.0581       & \textbf{0.0820} & 3.5\%  \\
                        & HR@10   & 0.0524  & 0.0676       & 0.0677       & 0.0699 & 0.0912 & {\ul 0.1043} & 0.0666       & 0.0819  & 0.0831  & 0.0828       & \textbf{0.1065} & 2.1\%  \\
                        & HR@20   & 0.076   & 0.0908       & 0.0968       & 0.1114 & 0.1209 & {\ul 0.1382} & 0.0879       & 0.1099  & 0.1150  & 0.1143       & \textbf{0.1409} & 1.9\%  \\
                        & NDCG@5  & 0.0247  & 0.0329       & 0.0322       & 0.0158 & 0.047  & {\ul 0.0579} & 0.0356       & 0.403   & 0.0407  & 0.0408       & \textbf{0.0603} & 4.1\%  \\
                        & NDCG@10 & 0.0296  & 0.0389       & 0.0391       & 0.0274 & 0.0552 & {\ul 0.0660} & 0.0415       & 0.481   & 0.0492  & 0.0488       & \textbf{0.0681} & 3.2\%  \\
                        & NDCG@20 & 0.0356  & 0.0448       & 0.0464       & 0.0378 & 0.0627 & {\ul 0.0745} & 0.0469       & 0.574   & 0.0577  & 0.0567       & \textbf{0.0759} & 1.9\%  \\
\hline
\multirow{6}{*}{ML-20m} & HR@5    & 0.1365  & 0.1305       & 0.1446       & 0.0655 & 0.1205 & 0.1380       & {\ul 0.1458} & 0.1325  & 0.1303  & 0.1367       & \textbf{0.1538} & 5.5\%  \\
                        & HR@10   & 0.2052  & 0.2016       & {\ul 0.2172} & 0.1312 & 0.1853 & 0.2070       & 0.2164       & 0.2022  & 0.2013  & 0.2071       & \textbf{0.2246} & 3.4\%  \\
                        & HR@20   & 0.2981  & 0.2996       & {\ul 0.3132} & 0.2251 & 0.2760 & 0.2997       & 0.3108       & 0.2994  & 0.2978  & 0.3021       & \textbf{0.3230} & 3.1\%  \\
                        & NDCG@5  & 0.0927  & 0.0858       & 0.0964       & 0.0347 & 0.0804 & 0.0927       & {\ul 0.0986} & 0.0899  & 0.0844  & 0.0918       & \textbf{0.1046} & 6.1\%  \\
                        & NDCG@10 & 0.1148  & 0.1086       & 0.1197       & 0.0558 & 0.1012 & 0.1149       & {\ul 0.1212} & 0.1121  & 0.1119  & 0.1144       & \textbf{0.1276} & 5.3\%  \\
                        & NDCG@20 & 0.1382  & 0.1333       & 0.1438       & 0.0794 & 0.1240 & 0.1382       & {\ul 0.1450} & 0.1334  & 0.1357  & 0.1383       & \textbf{0.1513} & 4.3\% \\
\bottomrule
\end{tabular}
\end{table*}

% \begin{table*}[htb]
% \small
% \centering
% \caption{Performance comparison of different methods on top-$k$ recommendation}
% \label{tab: mainresults}
% \begin{tabular}{c|c|cccc|ccc|ccc|c}
% \hline
% Dataset                 & Metric  & GRU4Rec & SASRec & BERT4Rec & CORE   & CL4Rec & ICLRec & DuoRec & A-Mixer & MSGIFSR & MiaSRec & Ours \\
% \hline
% \multirow{6}{*}{Beauty} & HR@5    & 0.0408  & 0.0508 & 0.0259   & 0.0331 & 0.0623 & 0.0664 & x      & 0.0589  & x       & 0.0524  & x    \\
%                         & HR@10   & 0.0623  & 0.0761 & 0.0406   & 0.0664 & 0.0877 & 0.0918 & x      & 0.8422  & x       & 0.0795  & x    \\
%                         & HR@20   & 0.0895  & 0.1057 & 0.0603   & 0.1071 & 0.1195 & 0.1252 & x      & 0.1154  & x       & 0.1125  & x    \\
%                         & NDCG@5  & 0.0273  & 0.0318 & 0.0169   & 0.0164 & 0.0440 & 0.048  & x      & 0.0403  & x       & 0.0362  & x    \\
%                         & NDCG@10 & 0.0342  & 0.0400 & 0.0216   & 0.0271 & 0.0521 & 0.0562 & x      & 0.0485  & x       & 0.0449  & x    \\
%                         & NDCG@20 & 0.0410  & 0.0474 & 0.0265   & 0.0373 & 0.0601 & 0.0646 & x      & 0.0563  & x       & 0.0532  & x    \\
% \hline
% \multirow{6}{*}{Sports} & HR@5    & 0.0210  & 0.0266 & 0.0104   & 0.0150 & 0.0338 & 0.0394 & x      & 0.0316  & x       & 0.0270  & x    \\
%                         & HR@10   & 0.0339  & 0.0412 & 0.0178   & 0.0342 & 0.0498 & 0.0553 & x      & 0.0472  & x       & 0.0435  & x    \\
%                         & HR@20   & 0.0527  & 0.0618 & 0.0302   & 0.0609 & 0.0723 & 0.0763 & x      & 0.0691  & x       & 0.0651  & x    \\
%                         & NDCG@5  & 0.0136  & 0.0158 & 0.0068   & 0.0072 & 0.0235 & 0.0276 & x      & 0.0212  & x       & 0.0180  & x    \\
%                         & NDCG@10 & 0.0178  & 0.0205 & 0.0091   & 0.0134 & 0.0287 & 0.0327 & x      & 0.0262  & x       & 0.0233  & x    \\
%                         & NDCG@20 & 0.0225  & 0.0256 & 0.0123   & 0.0201 & 0.0344 & 0.0380 & x      & 0.0318  & x       & 0.0288  & x    \\
% \hline
% \multirow{6}{*}{Toys}   & HR@5    & 0.0369  & 0.0489 & 0.0215   & 0.0338 & 0.0658 & 0.0792 & x      & 0.0607  & x       & 0.0581  & x    \\
%                         & HR@10   & 0.0524  & 0.0676 & 0.0319   & 0.0699 & 0.0912 & 0.1043 & x      & 0.0841  & x       & 0.0828  & x    \\
%                         & HR@20   & 0.0760  & 0.0908 & 0.0477   & 0.1114 & 0.1209 & 0.1382 & x      & 0.1119  & x       & 0.1143  & x    \\
%                         & NDCG@5  & 0.0247  & 0.0329 & 0.0138   & 0.0158 & 0.0470 & 0.0579 & x      & 0.0428  & x       & 0.0408  & x    \\
%                         & NDCG@10 & 0.0296  & 0.0389 & 0.0171   & 0.0274 & 0.0552 & 0.0660 & x      & 0.0503  & x       & 0.0488  & x    \\
%                         & NDCG@20 & 0.0356  & 0.0448 & 0.0211   & 0.0378 & 0.0627 & 0.0745 & x      & 0.0573  & x       & 0.0567  & x    \\
% \hline
% \multirow{6}{*}{Yelp}   & HR@5    & 0.0235  & 0.0403 & 0.0147   & 0.0523 & 0.0264 & x      & x      & x       & x       & 0.0571  & x    \\
%                         & HR@10   & 0.0396  & 0.0564 & 0.0264   & 0.0795 & 0.0425 & x      & x      & x       & x       & 0.0815  & x    \\
%                         & HR@20   & 0.0648  & 0.0797 & 0.0447   & 0.1137 & 0.0682 & x      & x      & x       & x       & 0.1160  & x    \\
%                         & NDCG@5  & 0.0149  & 0.0307 & 0.0092   & 0.0349 & 0.0168 & x      & x      & x       & x       & 0.0375  & x    \\
%                         & NDCG@10 & 0.0200  & 0.0359 & 0.0130   & 0.0436 & 0.0219 & x      & x      & x       & x       & 0.0454  & x    \\
%                         & NDCG@20 & 0.0263  & 0.0417 & 0.0176   & 0.0522 & 0.0284 & x      & x      & x       & x       & 0.0540  & x    \\
% \hline
% \end{tabular}
% \end{table*}


